HaloQuest: A Visual Hallucination Dataset for Advancing Multimodal Reasoning

Hallucination has been a major problem for large language models and remains a critical challenge when it comes to multimodality in which vision-language models (VLMs) have to deal with not just textual but also visual inputs. Despite rapid progress in VLMs, resources for evaluating and addressing multimodal hallucination are limited and mostly focused on evaluation. This work introduces HaloQuest, a novel visual question answering dataset that captures various aspects of multimodal hallucination such as false premises, insufficient contexts, and visual challenges. A novel idea from HaloQuest is to leverage synthetic images, apart from real ones, to enable dataset creation at scale. With over 7.7K examples spanning across a wide variety of categories, HaloQuest was designed to be both a challenging benchmark for VLMs and a fine-tuning dataset for advancing multimodal reasoning. Our experiments reveal that current models struggle with HaloQuest, with all open-source VLMs achieving below 36% accuracy. On the other hand, fine-tuning on HaloQuest significantly reduces hallucination rates while preserving performance on standard reasoning tasks. Our results discover that benchmarking with generated images is highly correlated (r=0.97) with real images. Last but not least, we propose a novel Auto-Eval mechanism that is highly correlated with human raters (r=0.99) for evaluating VLMs. In sum, this work makes concrete strides towards understanding, evaluating, and mitigating hallucination in VLMs, serving as an important step towards more reliable multimodal AI systems in the future.

==> sections/old_tables.tex <==



\begin{table}[t]
\begin{center}
\scalebox{0.8}{
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c }
\hline
\multicolumn{7}{c}{\cellcolor[HTML]{C0C0C0}\textit{\textbf{Zero-shot Evaluation with Benchmark Models}}}                                                                                                                                                         \\
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Model}} & \textbf{\# Param}          & \textbf{BLEU}                        & \textbf{CIDER}                       & \textbf{METEOR}                      & \textbf{Auto-Eval}      & \textbf{Human}          \\ \hline
{\color[HTML]{000000} LLaVA}                               & {\color[HTML]{000000} 13B} & {\color[HTML]{000000} \textbf{0.23}} & {\color[HTML]{000000} \textbf{1.15}} & {\color[HTML]{000000} \textbf{0.28}} & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
{\color[HTML]{000000} MiniGPT4}                            & {\color[HTML]{000000} 13B} & {\color[HTML]{000000} 0.08}          & {\color[HTML]{000000} 0.40}          & {\color[HTML]{000000} 0.19}          & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
{\color[HTML]{000000} BLIP2}                               & {\color[HTML]{000000} 12B} & {\color[HTML]{000000} 0.00}          & {\color[HTML]{000000} 0.06}          & {\color[HTML]{000000} 0.02}          & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
{\color[HTML]{000000} InstructBLIP}                        & {\color[HTML]{000000} 12B} & {\color[HTML]{000000} 0.00}          & {\color[HTML]{000000} 0.06}          & {\color[HTML]{000000} 0.02}          & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\ \hline
{\color[HTML]{000000} Open-flamingo}                       & {\color[HTML]{000000} 9B}  & {\color[HTML]{000000} 0.17}          & {\color[HTML]{000000} 0.31}          & {\color[HTML]{000000} 0.13}          & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
{\color[HTML]{000000} BLIP2}                               & {\color[HTML]{000000} 8B}  & {\color[HTML]{000000} 0.00}          & {\color[HTML]{000000} 0.06}          & {\color[HTML]{000000} 0.02}          & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
{\color[HTML]{000000} InstructBLIP}                        & {\color[HTML]{000000} 8B}  & {\color[HTML]{000000} 0.00}          & {\color[HTML]{000000} 0.06}          & {\color[HTML]{000000} 0.02}          & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
{\color[HTML]{000000} mPLUG-Owl2}                          & {\color[HTML]{000000} 8B}  & {\color[HTML]{000000} 0.00}          & {\color[HTML]{000000} 0.07}          & {\color[HTML]{000000} 0.02}          & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
{\color[HTML]{000000} mPLUG-Owl1}                          & {\color[HTML]{000000} 8B}  & {\color[HTML]{000000} \textbf{0.28}} & {\color[HTML]{000000} \textbf{1.16}} & {\color[HTML]{000000} \textbf{0.29}} & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\ \hline
{\color[HTML]{000000} Open-flamingo}                       & {\color[HTML]{000000} 3B}  & {\color[HTML]{000000} 0.16}          & {\color[HTML]{000000} 0.28}          & {\color[HTML]{000000} 0.13}          & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
OFA-huge                                                   & 1B                         & \textbf{0.18}                        & \textbf{0.65}                        & \textbf{0.20}                        &                         &                         \\ \hline
GPT-4                                                      &                            &                                      &                                      &                                      &                         &                         \\
Gemini                                                     &                            &                                      &                                      &                                      &                         &                         \\ \hline
\end{tabular}
}
\end{center}
\vspace{-0mm}
\caption{}
\label{tab:benchmark}
\vspace{-0mm}
\end{table}









==> tables/auto-eval-accuracy.tex <==
\begin{table}[t]
\centering
\caption{Detailed evaluation comparison by Auto-Eval. }
\scalebox{0.8}{
\begin{tabular}{l c c c c}
\toprule 
\textbf{Model (\# Param)} & \textbf{Human Eval}  & \textbf{Text-only} & \textbf{Basic Langfun} & \textbf{Langfun+reasoning}\\ 
\midrule
LLaVA (13B) \cite{llava} & 10.86 & 10.03 (98.19) & 10.69 (98.51) & \textbf{10.85 (98.6)} \\
MiniGPT4 (13B) \cite{minigpt4} & 18.42 & 39.80 (73.3) &  24.01 (82.56) & \textbf{25.16 (84.7)} \\
BLIP2 (12B) \cite{blip2} & 21.05 & 22.69 (94.40) & \textbf{22.20 (94.57)} & \textbf{22.53 (94.57)} \\
InstructBLIP (12B) \cite{instructblip} & 25.49 & 28.94 (95.23) &  \textbf{27.96 (95.88)} & 28.45 (95.39)  \\ 
\midrule
Open-flamingo (9B) \cite{openflamingo} & 13.82 & 16.11 (95.72) & \textbf{15.46 (96.38)} & 14.96 (95.88) \\
BLIP2 (8B) \cite{blip2} & 10.86 & \textbf{12.33 (96.54)} & 12.0 (96.21) & 11.84 (96.38)\\
InstructBLIP (8B) \cite{instructblip} & 25.00 & 28.12 (94.90) & \textbf{26.97 (95.72)} & 27.30 (95.39) \\
mPLUG-Owl2 (8B) \cite{mplug2} & 9.21 & 10.52 (96.71) & 10.52 (96.71) & \textbf{10.36 (96.87)} \\
mPLUG-Owl1 (8B) \cite{mplug1} & 9.70 &  \textbf{8.38 (98.68)} & 9.04 (98.35) & \textbf{8.71 (98.68)}\\ 
\midrule
Open-flamingo (3B) \cite{openflamingo} & 6.91 & 10.03 (96.21) & \textbf{8.05 (98.19)} & 8.22 (98.02) \\
OFA (1B) \cite{ofa} & 8.72 & 18.75 (89.63) &  \textbf{10.19 (97.20)} & 10.19 (96.87)\\
BEiT-3 (0.7B) \cite{beit3}& 35.86 & 41.44 (93.42) & \textbf{39.80 (94.73)} & 39.96 (94.57)\\ 
\midrule
GPT-4 \cite{gpt4v} & 65.79 & 70.06 (90.78) & 60.69 (87.66) & \textbf{64.3 (92.92)}\\
% Gemini Pro$^*$ \cite{gemini} & 46.96 & 49.57 & \\ 
\bottomrule
\end{tabular}
}
\label{tab:detailed-auto-eval}
\end{table}



==> tables/finetuning_details.tex <==

\begin{table}
    \centering
    \caption{Effect of training data on benchmark performance.  HaloQuest accuracy is measured with both human raters and with Auto-Eval, and VQA v2 performance is measured by exact match and broken down by question subtype, as is standard. Including HaloQuest training data effectively reduces hallucination rates, as shown by improved performance on the HaloQuest evaluation set.  Importantly, adding HaloQuest training data does not degrade performance on VQA v2, and in most cases helps.  These results show that HaloQuest is an effective dataset for reducing hallucination rates without sacrificing other model capabilities. $\ast$ represents situations when the machine-generated question-answer pairs are removed and only human-annotated question-answer pairs are reserved in the training set.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{llcccccc}
        \toprule
        \multirow{2}{*}{\textbf{Model (\# Param)}} & \multirow{2}{*}{\textbf{Training Data}} & \multicolumn{2}{c}{\textbf{HaloQuest}} & \multicolumn{4}{c}{\textbf{VQA v2}} \\
        \cmidrule(lr){3-4} \cmidrule(lr){5-8}
        & & \textbf{Human Eval} & \textbf{Auto-Eval} & \textbf{Overall} & \textbf{Binary} & \textbf{Number} & \textbf{Others} \\
        \midrule
        
        \multirow{2}{*}{BLIP2 (8B) \cite{blip2}} & VQA v2 & 11.18 & 12.34 & 70.50 & 87.04 & 52.42 & 59.94 \\
        & VQA v2 + HaloQuest$\ast$ & -- & 29.11 & 70.41 & 86.85 & \textbf{54.19} & 60.33 \\
        & VQA v2 + HaloQuest & \textbf{33.88} & \textbf{34.70} & \textbf{70.96} & \textbf{87.12} & 54.17 & \textbf{60.73} \\
        \midrule
        
        \multirow{2}{*}{mPLUG-Owl1 (8B) \cite{mplug2}} & VQA v2 & 9.70 & 9.54 & 74.17 & 89.75 & 57.31 & 64.45 \\
        & VQA v2 + HaloQuest$\ast$ & \textbf{--} & 4.22 & 74.49 & 89.81 & 58.60 & \textbf{64.91} \\
        & VQA v2 + HaloQuest & \textbf{25.82} & \textbf{29.11} & \textbf{74.92} & \textbf{90.04} & \textbf{58.73} & 64.90 \\
        \midrule

        \multirow{2}{*}{MiniGPT4 (8B) \cite{minigpt4}} & VQA v2 & 10.53 & 10.69 & 70.96 & 87.07 & 48.62 & 61.91 \\
        & VQA v2 + HaloQuest$\ast$ & -- & 23.19 & 71.13   & 87.39  & 51.60  & \textbf{61.94}  \\ 
        & VQA v2 + HaloQuest & \textbf{26.64} & \textbf{27.96} & \textbf{71.37}   & \textbf{87.84}  & \textbf{51.99}  & 61.90  \\ 
        \midrule
        \multirow{2}{*}{MiniGPT4 (13B) \cite{minigpt4}} & VQA v2 & 18.26 & 16.12 & 74.85 & 90.31 & 54.22 & 65.04 \\
        & VQA v2 + HaloQuest$\ast$ & -- & 32.40 & 74.80 & 90.22  & 56.40  & 65.37  \\ 
        & VQA v2 + HaloQuest & \textbf{35.53} & \textbf{40.13} & \textbf{74.87} & \textbf{90.78}  & \textbf{56.73}  & \textbf{65.38}  \\ 
        \bottomrule
    \end{tabular}
    }
    \label{tab:finetuning_details}
\end{table}

